Web data mining for public health purposes

For a long time, public health events, such as disease incidence or vaccination activity, have been monitored to keep track of the health status of the population, allowing to evaluate the effect of public health initiatives and to decide where resources for improving public health are best spent. This thesis investigates the use of web data mining for public health monitoring, and makes contributions in the following two areas: New approaches for predicting public health events from web mined data, and novel applications of web mined data for public health monitoring.

==> introduction/Machine_learning_for_prediction.tex <==
%3) Machine learning approaches
%3.1) linear models
%3.2) gaussian processes as nonlinear extenstions of linear models
%3.3) regression trees and online learning



==> introduction/looking_ahead.tex <==
\section{Perspectives and future work}\label{sec:looking_ahead}


The previous sections have given us a overview of the motivation for using frequency data for prediction, how it started and where it is today. 

\textcolor{red}{make the sections fit together by describing how we see can see the importance of these systems based on the current status presented in the first section and the methods described afterwards.}


In the following section we will touch upon what might be the future work for query frequency based prediction methods. 

\subsection{Using media debates for early detection}
% different types of events, infectious diseases vs vaccination uptake or antibiotics.
% the use of media monitoring for early detection of change in vaccination attitude.

So far we have not distinguished between the different types of events being predicted, but there is at least two categories worth considering: \textit{conscious} and \textit{unconscious}. 

\textcolor{red}{find other words than conscious and unconscious}

\paragraph{Conscious} This category includes conscious events such as vaccination. For the conscious events there might be a chance to improve early detection of changes by considering data sources that might indicate changes in the public opinion.

\paragraph{Unconscious} Those events include infectious diseases or emergency hospital admissions. These are events that we as persons do not have full control over, our behavior do affect the risk of contracting a disease or getting admitted to a hospital, but it is generally speaking not something that is a conscious choice. 
\\
\\
For early detection of changing trends the conscious events are of special interest. Media has previously been identified as agenda-setting\cite{mccombs2009news}, meaning that coverage in the media affects the salience of topics in the public agenda, i.e. peoples perception of the world. We have in our work been analyzing media coverage of vaccination uptake, section \ref{cha:new_media_vacc}, both for the measles, mumps and rubella (MMR) vaccine and human papillomavirus (HPV) vaccine. 

For the case of the MMR vaccine and media coverage, section \ref{sec:mmr_media}, we observed for the period 1998-2004 a positive correlation between positive media coverage and MMR vaccination uptake of the first vaccine, and between neutral media coverage and first vaccine. For the following period 2005-2014 we observe no correlation. The correlation coincides with the debate about the MMR vaccine and autism, and the fact that the media in this period contains both negative and positive media coverage might explain the effect. Studies about the importance of integration in the European Union across countries have reported similar observations, namely that in countries where the political elite disagreed there was a relationship between media coverage and the public opinion, while in countries where the political elite agreed there was no relationship\cite{mccombs2009news}. Similarly we observed no significant correlation between the HPV and media coverage for the period January 2009 - June 2013 there is no correlation between media coverage and HPV vaccination uptake, while for the period Juli 2013 to January 2016 there is a correlation, again this corresponds to a change in the media coverage. 

In both cases the correlations are small, and for the MMR vaccination uptake it was only observed for annotated media, indicating that media is not a strong enough predictor, but it might be a useful tool for identifying changing points that can be early warnings for changes in the vaccination uptake. If it is indeed the amount of disagreement that controls the power of the media, then it would be necessary to apply stance or sentiment detection in order for the detection to work. 

\subsection{Evaluation methods for query frequency predictions}
% avoiding errors:
%	reducing suprious correlations
%	automatically updating models based current input
%	new evaluation methods

Work on usage of web search frequencies for prediction of health events focuses on either reducing the prediction error of previous prediction problems or using web search frequencies for new problems. But in all cases the evaluation metric is typically the same, i.e. prediction error or correlation, not taking into account that many of these signals are often relatively stable. The influenza season is for example very seasonal and the prediction accuracy in non-epidemic periods are of only limited relevance, illustrated by the fact that Denmark only monitors influenza activity from week 40 to week 20 the following year. 

\subsection{Improving query selection}

Using correlation for query selection is vulnerable to changes in search behavior, for example introduction of new terms such as ``avian flu'' or ``swine flu''. Relying on correlation for query selection has the inherent problem that emerging trends will not be discovered before there are sufficient historic data. Perhapses social media and news media could be used for detecting changes in vocabulary use that could be used for updating the query terms included in the models. Combining the introduction of new query terms with an online learning approach, as we did in \cite{www17}, would mean that as the new terms grows more common they would automatically receive a larger weight in the prediction model. 





